MorphStream: Scalable Processing of Transactions over Streams on Multicores

Transactional Stream Processing Engines (TSPEs) form the backbone of modern stream applications handling shared mutable states. Yet, the full potential of these systems, specifically in exploiting parallelism and implementing dynamic scheduling strategies, is largely unexplored. We present MorphStream, a TSPE designed to optimize parallelism and performance for transactional stream processing on multicores. Through a unique three-stage execution paradigm (i.e., planning, scheduling, and execution), MorphStream enables dynamic scheduling and parallel processing in TSPEs. Our experiment showcased MorphStream outperforms current TSPEs across various scenarios and offers support for windowed state transactions and non-deterministic state access, demonstrating its potential for broad applicability.

==> Experiments/DetailedWorkloads.tex <==
 
\emph{Workload 1: SL}
is described earlier in Figure~\ref{fig:TPG} in Section~\ref{subsec:construction}.
Two tables of 100k account and asset records are kept as the shared mutable states.
The \emph{Transfer} transaction has a transaction length $l$ of 4, i.e., transfer from a pair of accounts and assets to another pair. 
In particular, the state access per operation ($r$) is 2, i.e., updating a user account requires a read from another user account.
The \emph{Deposit} transaction has a $l$ of 2 to update a pair of accounts and assets. Each operation is write-only, and the state access per operation $r$ is 1.

\emph{Workload 2: GS}
represents a workload scenario where an application modifies large shared mutable states.
% Random generated \emph{Sum} transactions are to be generated for each input event.
% It processes input events that involve reading a subset of the values of selected states.
GS maintains a table of 100k records.
% as the shared mutable states.
\emph{Sum} transactions may be generated during the processing of each input event.
% \emph{Sum} transactions are read-only in the original implementation.
\emph{Sum} transactions processes requests that read from selected states, performs summation among the obtained state values, followed by a write to the first state it reads. By default, its $l$ is 1 and $r$ is 10.

\curry{\emph{Workload 3: TP}
represents a toll processing application, which calculates the toll for each reported vehicle based on the congestion status of the road . 
The road congestion status are shared among all operations with two mutable table. One to record the average road speed and the other to count the number of unique vehicles.
\emph{Toll} transactions processes position report of a vehicle that update related records(road speed and count of unique vehicles), and computes the toll by a read to the congestion status. By default, its $l$ is 2 and $r$ is 1.}

\curry{\emph{Workload 4: OB}
stands for an Online Bidding system. All operations share a table with 10k unique bid items.
\emph{Bid} transaction reduces the quantity of its requested item, with the condition that bid price is not less than the asking price and the item has a sufficient quantity, otherwise the request is rejected.
\emph{Alert} transaction modify the asking price of the requested item list.
\emph{Top} transaction increment the quantity of items list by the given value.
By default, the $l$ and $r$ of bid transaction is 1 and 1 respectively. And alert transaction and top transaction are identical, their l is 5 and r is 1.
}

==> vldb_block.tex <==
%%% do not modify the following VLDB block %%
%%% VLDB block start %%%
\pagestyle{\vldbpagestyle}
\begingroup\small\noindent\raggedright\textbf{PVLDB Reference Format:}\\
\vldbauthors. \vldbtitle. PVLDB, \vldbvolume(\vldbissue): \vldbpages, \vldbyear.\\
\href{https://doi.org/\vldbdoi}{doi:\vldbdoi}
\endgroup
\begingroup
\renewcommand\thefootnote{}\footnote{\noindent
This work is licensed under the Creative Commons BY-NC-ND 4.0 International License. Visit \url{https://creativecommons.org/licenses/by-nc-nd/4.0/} to view a copy of this license. For any use beyond those covered by this license, obtain permission by emailing \href{mailto:info@vldb.org}{info@vldb.org}. Copyright is held by the owner/author(s). Publication rights licensed to the VLDB Endowment. \\
\raggedright Proceedings of the VLDB Endowment, Vol. \vldbvolume, No. \vldbissue\ %
ISSN 2150-8097. \\
\href{https://doi.org/\vldbdoi}{doi:\vldbdoi} \\
}\addtocounter{footnote}{-1}\endgroup
%%% VLDB block end %%%

%%% do not modify the following VLDB block %%
%%% VLDB block start %%%
\ifdefempty{\vldbavailabilityurl}{}{
\vspace{.3cm}
\begingroup\small\noindent\raggedright\textbf{PVLDB Artifact Availability:}\\
The source code, data, and/or other artifacts have been made available at \url{\vldbavailabilityurl}.
\endgroup
}
%%% VLDB block end %%%

==> vldb_prefix.tex <==
%% The following content must be adapted for the final version
% paper-specific
\newcommand\vldbdoi{XX.XX/XXX.XX}
\newcommand\vldbpages{XXX-XXX}
% issue-specific
\newcommand\vldbvolume{14}
\newcommand\vldbissue{1}
\newcommand\vldbyear{2020}
% should be fine as it is
\newcommand\vldbauthors{\authors}
\newcommand\vldbtitle{\shorttitle} 
% leave empty if no availability url should be set
\newcommand\vldbavailabilityurl{https://github.com/intellistream/TStream}
% whether page numbers should be shown or not, use 'plain' for review versions, 'empty' for camera ready
\newcommand\vldbpagestyle{plain} 
